Cross-Context Backdoor Attacks against Graph Prompt Learning

Graph Prompt Learning (GPL) bridges significant disparities between pretraining and downstream applications to alleviate the knowledge transfer bottleneck in real-world graph learning. While GPL offers superior effectiveness in graph knowledge transfer and computational efficiency, the security risks posed by backdoor poisoning effects embedded in pretrained models remain largely unexplored. Our study provides a comprehensive analysis of GPL's vulnerability to backdoor attacks. We introduce \textit{CrossBA}, the first cross-context backdoor attack against GPL, which manipulates only the pretraining phase without requiring knowledge of downstream applications. Our investigation reveals both theoretically and empirically that tuning trigger graphs, combined with prompt transformations, can seamlessly transfer the backdoor threat from pretrained encoders to downstream applications. Through extensive experiments involving 3 representative GPL methods across 5 distinct cross-context scenarios and 5 benchmark datasets of node and graph classification tasks, we demonstrate that \textit{CrossBA} consistently achieves high attack success rates while preserving the functionality of downstream applications over clean input. We also explore potential countermeasures against \textit{CrossBA} and conclude that current defenses are insufficient to mitigate \textit{CrossBA}. Our study highlights the persistent backdoor threats to GPL systems, raising trustworthiness concerns in the practices of GPL techniques.

==> 9-rebuttal.tex <==
\section{Rebuttal}


By increasing the number of nodes in the trigger graph, we observe whether the trigger graph can be more easily detected using the defense algorithm ? 

Response: We have tested with the defense algorithm (Node Pruning), the variation of the attack success rate with different number of nodes set in the attached trigger graph in XXXX (Figure or Table). We show XXXX increasing the number of trigger nodes does not significantly change the attack success rate. This indicates that increasing the trigger nodes does not necessarilly indicate an easier defense against the proposed backdoor attack. The reason is attributed to XXXX. 







==> table/relatedwork-cross.tex <==
\begin{table}[h]
\centering
\footnotesize
\caption{Summary  about the cross-context scenarios.}
\label{tab:related work}
\resizebox{\columnwidth}{!}{%
\begin{tabular}{@{}c|c|c|c|c|c@{}}
\toprule
GPL Method & \makecell{Cross \\ Distribution} & \makecell{Cross \\ Class} & \makecell{Cross \\ Dataset} & \makecell{Cross \\ Domain} & \makecell{Cross \\ Task} \\ 
\midrule
ProG \cite{allinone}  & \checkmark  &   & \checkmark  & \checkmark  & \checkmark  \\
GraphPrompt \cite{graphprompt}  & \checkmark  &   & \checkmark &   & \checkmark  \\
VNT \cite{VNT}  &  \checkmark  &\checkmark  &   &   &  \\
GPF-Plus \cite{DBLP:journals/corr/abs-2209-15240}  &  \checkmark  &   &   & \checkmark  &  \\
% ULTRA-DP \cite{DBLP:journals/corr/abs-2310-14845}& \checkmark &   &  &   &  \\
\textbf{CrossBA (ours)} & \checkmark  & \checkmark  & \checkmark  & \checkmark  & \checkmark \\
\bottomrule
\end{tabular}
}
\end{table}
